The Variability of the Star Formation Rate in Galaxies: I. Star Formation Histories Traced by EW(H$\alpha$) and EW(H$\delta_A$)

To investigate the variability of the star formation rate (SFR) of galaxies, we define a star formation change parameter, SFR$_{\rm 5Myr}$/SFR$_{\rm 800Myr}$ which is the ratio of the SFR averaged within the last 5 Myr to the SFR averaged within the last 800 Myr. We show that this parameter can be determined from a combination of H$\alpha$ emission and H$\delta$ absorption, plus the 4000 A break, with an uncertainty of $\sim$0.07 dex for star-forming galaxies. We then apply this estimator to MaNGA galaxies, both globally within Re and within radial annuli. We find that galaxies with higher global SFR$_{\rm 5Myr}$/SFR$_{\rm 800Myr}$ appear to have higher SFR$_{\rm 5Myr}$/SFR$_{\rm 800Myr}$ at all galactic radii, i.e. that galaxies with a recent temporal enhancement in overall SFR have enhanced star formation at all galactic radii. The dispersion of the SFR$_{\rm 5Myr}$/SFR$_{\rm 800Myr}$ at a given relative galactic radius and a given stellar mass decreases with the (indirectly inferred) gas depletion time: locations with short gas depletion time appear to undergo bigger variations in their star-formation rates on Gyr or less timescales. In Wang et al. (2019) we showed that the dispersion in star-formation rate surface densities $\Sigma_{\rm SFR}$ in the galaxy population appears to be inversely correlated with the inferred gas depletion timescale and interpreted this in terms of the dynamical response of a gas-regulator system to changes in the gas inflow rate. In this paper, we can now prove directly with SFR$_{\rm 5Myr}$/SFR$_{\rm 800Myr}$ that these effects are indeed due to genuine temporal variations in the SFR of individual galaxies on timescales between $10^7$ and $10^9$ years rather than possibly reflecting intrinsic, non-temporal, differences between different galaxies.

==> makefile <==
SOURCE = ms

.SUFFIXES:	.aux .dvi .ps .tex

# edit and process the .tex file
default:	twice ps 
#gv

main:		$(SOURCE).aux
			latex $(SOURCE)
dvi:		$(SOURCE).dvi
ps:			$(SOURCE).ps
once:
			latex $(SOURCE)
twice:		once once
			latex $(SOURCE)
bib:		
			bibtex $(SOURCE)

x:			$(SOURCE).dvi
			xdvi -geometry +0+0 -s 8 -bg white -fg black \
			-expert -hush $(SOURCE).dvi &
gv:			$(SOURCE).ps
			gv $(SOURCE).ps &


.dvi.ps:
			dvips -f $< > $(SOURCE).ps
.tex.aux:
			latex $(SOURCE)	# create .aux file from $<
.tex.dvi:
			latex $<	# create .dvi file from $<

clean:	
			rm -f *~ *.log *.dvi *.aux *.blg  *.lof *.lot *.toc *.bbl *~ 
cleanest:	
			rm -f *~ *.log *.dvi *.ps *.aux *.toc *.bbl *.blg *.lot


